Quadruped Capturability and Push Recovery via a Switched-Systems Characterization of Dynamic Balance

This paper studies capturability and push recovery for quadrupedal locomotion. Despite the rich literature on capturability analysis and push recovery control for legged robots, existing tools are developed mainly for bipeds or humanoids. Distinct quadrupedal features such as point contacts and multiple swinging legs prevent direct application of these methods. To address this gap, we propose a switched systems model for quadruped dynamics, and instantiate the abstract viability concept for quadrupedal locomotion with a time-based gait. Capturability is characterized through a novel specification of dynamically balanced states that addresses the time-varying nature of quadrupedal locomotion and balance. A linear inverted pendulum (LIP) model is adopted to demonstrate the theory and show how the newly developed quadrupedal capturability can be used in motion planning for quadrupedal push recovery. We formulate and solve an explicit model predictive control (EMPC) problem whose optimal solution fully characterizes quadrupedal capturability with the LIP. Given this analysis, an optimization-based planning scheme is devised for determining footsteps and center of mass references during push recovery. To validate the effectiveness of the overall framework, we conduct numerous simulation and hardware experiments. Simulation results illustrate the necessity of considering dynamic balance for quadrupedal capturability, and the significant improvement in disturbance rejection with the proposed strategy. Experimental validations on a replica of the Mini Cheetah quadruped demonstrate an up to 100% improvement as compared with state-of-the-art.

==> Quadrupedal Push Recovery_arXiv/newcommands.tex <==
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\theoremstyle{definition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{property}{Property}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
% \theoremstyle{remark}
\renewcommand{\baselinestretch}{1.2} 

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\DeclareFontFamily{U}{jkpmia}{}
\DeclareFontShape{U}{jkpmia}{m}{it}{<->s*jkpmia}{}
\DeclareFontShape{U}{jkpmia}{bx}{it}{<->s*jkpbmia}{}
\DeclareMathAlphabet{\mathfrak}{U}{jkpmia}{m}{it}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\Min}{Minimize }
\DeclareMathOperator*{\proj}{proj}
\DeclareMathOperator*{\modd}{mod}
\DeclareMathOperator{\arccot}{arccot}
\DeclareMathOperator{\blkdiag}{Blkdiag}
\DeclareMathOperator{\cvxhull}{Convhull}
\DeclareMathOperator{\dt}{dt}
\DeclareMathOperator{\ddt}{\frac{d}{dt}}
\DeclareMathOperator{\dtau}{d\tau}
% COMMANDS\newcommand{\Tt}{{\cal T}}
\DeclareMathOperator{\Pre}{Pre}
\DeclareMathOperator{\PRE}{PRE}
\newcommand{\Hh}{{\mathbf H}}
\newcommand{\ttau}{{ \boldsymbol \tau}}
\newcommand{\llambda}{{ \boldsymbol \lambda}}
\newcommand{\LLambda}{{ \boldsymbol \Lambda}}
\newcommand{\xxi}{{ \boldsymbol \xi}}
\newcommand{\Ja}{{\mathbf J}}
\newcommand{\w}{{\mathbf w}}
\newcommand{\Cs}{{\boldsymbol{\cal C}}}
\newcommand{\Ff}{{\mathbf F}}
\newcommand{\Ga}{{\mathbf G}}
\newcommand{\Sl}{{\mathbf S}}
\newcommand{\Tt}{{\mathbf T}}
\newcommand{\x}{{\mathbf x}}
\newcommand{\Xx}{{\mathbf X}}
\newcommand{\Uu}{{\mathbf U}}
\newcommand{\Aa}{{\mathbf A}}
\newcommand{\Bb}{{\mathbf B}}
\renewcommand{\u}{{\mathbf u}}
\newcommand{\Pf}{{\mathbf P}}
\newcommand{\Bx}{\boldsymbol{\mathcal{B}}}
\newcommand{\Bxb}{\bar{\boldsymbol{\mathcal{B}}}}
\newcommand{\sigmaa}{\boldsymbol{\sigma}}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\Xb}{\boldsymbol{\cal X}}
\newcommand{\Zb}{\boldsymbol{\cal Z}}
\newcommand{\Vb}{\boldsymbol{\cal V}}
\newcommand{\Ub}{\boldsymbol{\cal U}}
\renewcommand{\t}{\mathbf{t}}
\renewcommand{\o}{\mathbf{o}}
\renewcommand{\c}{\mathbf{c}}
\newcommand{\Cc}{\mathbf{C}}
\newcommand{\so}{\emph{SO}(3)}
\newcommand{\cone}{{\cal F C}}
\newcommand{\ys}{\mathsf{y}}
\newcommand{\xs}{x_{\mathtt{s}}}
\newcommand{\xsa}{x_{\mathtt{s},1}}
\newcommand{\xsb}{x_{\mathtt{s},2}}
\newcommand{\xsc}{x_{\mathtt{s},3}}
\newcommand{\xsd}{x_{\mathtt{s},4}}
\newcommand{\xf}{x_{\mathtt{f}}}
\newcommand{\xfa}{x_{\mathtt{f},1}}
\newcommand{\xfb}{{\mathbf x}^\text{fb}}
\newcommand{\xfc}{x_{\mathtt{f},3}}
\newcommand{\xfd}{x_{\mathtt{f},4}}
\newcommand{\xfe}{x_{\mathtt{f},5}}
\newcommand{\xff}{x_{\mathtt{f},6}}
\newcommand{\dxs}{\dot{x}_{\mathtt{s}}}
\newcommand{\dxf}{\dot{x}_{\mathtt{f}}}
% \renewcommand{\k}{\mathfrak{k}}
\newcommand{\gr}{\mathtt{g}}
\newcommand{\hz}{\mathtt{h}}
\newcommand{\Id}{\mathbf{I}}
\newcommand{\Ie}{\mathtt{I}}

% \newcommand{\m}{\mathfrak{m}}
% \renewcommand{\l}{\mathfrak{l}}
\newcommand{\h}{\mathbf{h}}
\newcommand{\pinv}{\dagger}
\newcommand{\y}{\mathbf{y}}%
\newcommand{\sA}{A_o}%
\newcommand{\sB}{B_o}
\newcommand{\sC}{C_o}
\newcommand{\sD}{D_o}
\renewcommand{\b}[1]{\overline{#1}}
\newcommand{\diag}{\mbox{diag}}
\newcommand{\im}{\mathbf{i}}
\newcommand{\re}{\mathbf{Re}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\p}{{\mathbf p}}%
\newcommand{\q}{{\mathbf q}}%
\newcommand{\e}{{\mathbf e}}%
\newcommand{\R}{\mathbb{R}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\field}{\mathbb{F}}
\newcommand{\End}{\mbox{End}}
\newcommand{\Frames}[1]{\mathcal{F}_{#1}}
\newcommand{\Btab}{\mathrm{Stab}}
\newcommand{\Bpan}{\mbox{span}}
\newcommand{\Proj}{\Pi}
\newcommand{\trace}{\mathrm{trace}}
\newcommand{\GL}{\lieg{GL}}
\newcommand{\Aff}{\mathrm{Aff}}
\newcommand{\Orb}{\mathrm{Orb}}
\newcommand{\group}{\mathsf}
\newcommand{\Lie}{\mathrm{Lie}}
\newcommand{\Lor}{\mathsf{Lor}}
\newcommand{\ILor}{\mathsf{ILor}}
\newcommand{\Gal}{\mathsf{Gal}}
\newcommand{\IGal}{\mathsf{IGal}}
\newcommand{\omegaup}{\omega^\uparrow}
\newcommand{\omegadown}{\omega^\downarrow}
\newcommand{\mbf}{\mathbf}
\newcommand{\nssym}[1]{\,{#1}\,}
\newcommand{\T}{\mathbf{T}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\Na}{\mathbb{N}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\Bt}{\boldsymbol{\B}}
\newcommand{\vr}{v^{r}}
\newcommand{\qr}{q^{r}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Xf}{\mathcal{X}_\text{free}}
\newcommand{\Xo}{\mathcal{X}_\text{obs}}
\newcommand{\Xg}{\mathcal{X}_\text{goal}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\Ww}{\mathbf{W}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\Z}{\mathcal{Z}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\M}{\mathcal{M}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\Pj}{\mathbb{P}}
% \newcommand{\Po}{\mathcal{P}_\text{obs}}
% \newcommand{\Pg}{\mathcal{P}_\text{goal}}
% \newcommand{\Uo}{\mathcal{U}_\text{obs}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\Reach}{\mathcal{R}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\Qc}{\mathbf{Q}}
\newcommand{\Rc}{\mathbf{R}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Ns}{\mathfrak{N}}
\renewcommand{\H}{\mathcal{H}}
\renewcommand{\b}[1]{\overline{#1}}
\newcommand{\la}{\leftarrow}
\newcommand{\case}[1]{\begin{cases}#1\end{cases}}
\newcommand{\ar}[1]{\left[\begin{array}#1\end{array}\right]}
\newcommand{\al}[1]{\begin{align}#1\end{align}}
\newcommand{\eq}[1]{\begin{equation}#1\end{equation}}
\newcommand{\ald}[1]{\begin{aligned}#1\end{aligned}}
\newcommand{\ra}{\Rightarrow}
\newcommand{\eqn}[1]{\begin{equation*}#1\end{equation*}}
\newcommand{\aln}[1]{\begin{align*}#1\end{align*}}
\newcommand{\subeq}[1]{\begin{subequations}#1\end{subequations}}
\newcommand{\st}{\text{s.t. }}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\tb}[1]{\textcolor{blue}{#1}}
\newcommand{\CIS}{\mathcal{C}}
\newcommand{\qfb}{\q^\text{fb}}
\newcommand{\qj}{\q^\text{J}}
\newcommand{\qp}{\q^\text{p}}
\newcommand{\qR}{\q^\text{R}}
\newcommand{\In}{{\mathbf 1}}
\newcommand{\g}{\mathbf g}
\newcommand{\omegaa}{\boldsymbol{\omega}}
\newcommand{\f}{\mathbf f}
\newcommand{\Eb}{\mathbf E}
\newcommand{\z}{\mathbf z}
\newcommand{\Uf}{\boldsymbol{\U}}
\renewcommand{\v}{\mathbf v}
\newcommand{\psii}{\boldsymbol{\psi}}
\newcommand{\Ca}{{\cal C}}
\newcommand{\Vvv}{{\mathbf V}}
\newcommand{\Rx}{{\mathscr {R}}}
\newcommand{\Cx}{{\mathscr {C}}}


==> Quadrupedal Push Recovery_arXiv/packages.tex <==
\usepackage[margin=1in]{geometry}
\usepackage{hyperref}
\usepackage{times,multirow,caption,float,url}
\usepackage{enumitem}
\usepackage{wrapfig}
\usepackage{graphicx}
\usepackage{epsfig,xspace,layout}
\usepackage{subfigure}
\usepackage{color}
\usepackage{amsfonts}
\usepackage{times}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{rotating}
\usepackage{amsthm}
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{mathrsfs}
\usepackage{caption}
\usepackage{subfigure}
\usepackage{mathtools}
\usepackage{makeidx}
\usepackage{multirow} 
\usepackage{dblfloatfix}
\usepackage{threeparttable}
\usepackage{dsfont}
\usepackage[font={small}]{caption}
\usepackage{cleveref}
% \usepackage{algorithm}
\usepackage[linesnumbered,algoruled,boxed,lined]{algorithm2e}
\usepackage{tikz}
\usetikzlibrary{shapes,arrows,positioning,calc}
\usepackage{siunitx}
\sisetup{load-configurations = abbreviations}
\usepackage{cite}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{siunitx}
\usepackage[title]{appendix}

